Intermittent Demand Forecasting with Renewal Processes

Intermittency is a common and challenging problem in demand forecasting. We introduce a new, unified framework for building intermittent demand forecasting models, which incorporates and allows to generalize existing methods in several directions. Our framework is based on extensions of well-established model-based methods to discrete-time renewal processes, which can parsimoniously account for patterns such as aging, clustering and quasi-periodicity in demand arrivals. The connection to discrete-time renewal processes allows not only for a principled extension of Croston-type models, but also for an natural inclusion of neural network based models---by replacing exponential smoothing with a recurrent neural network. We also demonstrate that modeling continuous-time demand arrivals, i.e., with a temporal point process, is possible via a trivial extension of our framework. This leads to more flexible modeling in scenarios where data of individual purchase orders are directly available with granular timestamps. Complementing this theoretical advancement, we demonstrate the efficacy of our framework for forecasting practice via an extensive empirical study on standard intermittent demand data sets, in which we report predictive accuracy in a variety of scenarios that compares favorably to the state of the art.

==> head.tex <==
\usepackage{array}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{booktabs}
% \usepackage{xcolor}
\usepackage{listings}
\usepackage{datetime}
\usepackage{hyperref}
\usepackage{natbib}
\usepackage{csquotes}
\usepackage{natbib}
\usepackage{adjustbox}
\usepackage[figuresright]{rotating}

%\usepackage{xtab}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{multirow}
\usepackage{subfigure}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage[ruled]{algorithm2e}
\usepackage{color}
\usepackage{stmaryrd}
\usepackage{booktabs}
% \usepackage[dvipsnames]{xcolor}
\usepackage{enumitem}

\newcommand{\ddx}{\frac{d}{dx}}  % derivative 
\newcommand{\dr}[1]{\dfrac{\partial}{\partial{#1}}} % partial derivative
\newcommand{\ddr}[2]{\dfrac{\partial{#1}}{\partial{#2}}} % partial
\newcommand{\ex}[1]{\mathbb{E}\left[ #1 \right]}  % mathematical expectation
\newcommand{\exs}[1]{\mathbb{E}[ #1 ]}  % mathematical expectation
\newcommand{\varn}[1]{\mathbb{V}[#1]}  % variance
\newcommand{\IR}{\mathbb{R}}  % Real numbers
\newcommand{\IP}[1]{\mathbb{P}\{#1\}}  % probability
\newcommand{\PR}[1]{\mathbb{P}\{#1\}}  % also probability
\newcommand{\HH}{\mathcal{H}}  % calligraphic H, often a filtration
\newcommand{\DD}{\mathcal{D}}  % calligraphic D, often data
\newcommand{\ZZ}{\mathcal{Z}}  % calligraphic Z, often set of latent variables
\newcommand{\II}[1]{\mathcal{I}_{#1}}  % calligraphic I with subscript, often an index set
\newcommand{\indf}[1]{\llbracket #1 \rrbracket}
% \newcommand{\EWMA}{\textit{EWMA}}  % 
% \newcommand{\ARIMA}{\textit{ARIMA}}  % 
\renewcommand{\b}[1]{\mathbf{#1}}  % easy boldface in math
\newcommand{\eg}{\emph{e.g.}}  % fancy e.g.
\newcommand{\ie}{\emph{i.e.}}  % fancy i.e.
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
%some matrices,
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bPhi}{\mathbf{\Phi}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bDh}{\mathbf{D}^{\frac{1}{2}}}
\newcommand{\bDmh}{\mathbf{D}^{-\frac{1}{2}}}
\newcommand{\bDE}{\mathbf{\Delta}}
\newcommand{\bDEh}{\mathbf{\Delta}^{\frac{1}{2}}}
\newcommand{\bDEmh}{\mathbf{\Delta}^{-\frac{1}{2}}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bPsi}{\mathbf{\Psi}}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\obs}{y} 

\newcommand{\fhalf}{\frac{1}{2}}
\newcommand{\mroot}[1]{{#1}^{\frac{1}{2}}}

\newcommand{\etal}{{\em et al.}}
\newcommand{\ARIMA}{\text{ARIMA}}
\newcommand{\LSTM}{\text{LSTM}}
\newcommand{\EWMA}{\text{EWMA}}


\newcommand{\distPo}[1]{\mathcal{PO}\left(#1\right)}

\newcommand{\todo}[1]{{\color{red} {\em TODO: #1}}}  % easy todo notes
\newcommand{\tocite}[1]{{\color{teal} {\em CIT NEEDED: #1}}}  % easy todo notes

\newtheorem{defn}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}

\newcommand{\colr}[1]{\textcolor{red}{#1}}  
\newcommand{\colb}[1]{\textcolor{blue}{#1}}
\newcommand{\colg}[1]{\textcolor{green}{#1}}



==> table/tab_dtrp_results_bak.tex <==
\begin{sidewaystable}
\label{tab:results_dtrp}
\centering
\caption{Experiment results for discrete-time models with Car Parts and Auto data sets}
% \begin{adjustbox}{angle=90}
% \begin{adjustwidth}{0in}{0in}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{3cm}p{8cm}cccccccc}
\toprule
Data Set  & Model         &     P50 Loss            &         P90 Loss        &  MAAPE                   &   MASE                     &  MAPE                      &             sMAPE         &   RMSE                        & RMSSE                       \\
\midrule
\multirow{16}{*}{\textbf{Car Parts}}
& All Zeros               &  N/A                    &  N/A                    &  {\bf 0.785             }&  {\bf 1.288               }&  1.000                     &  2.000                    &   1.513                       & 1.406                       \\
& Croston    \cCro        &  N/A                    &  N/A                    &  {\bf 1.181             }&  1.497                     &  0.568                     &  {\bf 1.604              }&   1.372                       & 1.307                       \\
& SBA        \cSBA        &  N/A                    &  N/A                    &  1.182                   &  1.489                     &  0.571                     &  1.607                    &   1.368                       & 1.301                       \\
& TSB        \cTSB        &  N/A                    &  N/A                    &  1.190                   &  1.446                     &  0.580                     &  1.615                    &   1.362                       & 1.278                       \\
& Static G-Po    \cCro    &  0.750 $\pm$ 0.002      &  0.638 $\pm$ 0.000      &  1.194 $\pm$ 0.000       &  1.554 $\pm$ 0.000         &  0.583 $\pm$ 0.000         &  1.608 $\pm$ 0.000        &   1.410 $\pm$ 0.001           & 1.345 $\pm$ 0.000           \\
& Static G-NB    \cSny    &  0.718 $\pm$ 0.001      &  0.713 $\pm$ 0.001      &  1.182 $\pm$ 0.000       &  1.624 $\pm$ 0.002         &  {\bf 0.538 $\pm$ 0.001   }&  {\bf 1.583 $\pm$ 0.000  }&   1.434 $\pm$ 0.000           & 1.366 $\pm$ 0.001           \\
& EWMA G-Po      \cShen   &  0.716 $\pm$ 0.002      &  0.791 $\pm$ 0.004      &  1.204 $\pm$ 0.000       &  1.552 $\pm$ 0.001         &  0.634 $\pm$ 0.001         &  1.663 $\pm$ 0.000        &   1.438 $\pm$ 0.001           & 1.363 $\pm$ 0.000           \\
& EWMA G-NB               &  0.711 $\pm$ 0.001      &  0.800 $\pm$ 0.000      &  1.204 $\pm$ 0.000       &  1.551 $\pm$ 0.001         &  0.635 $\pm$ 0.001         &  1.663 $\pm$ 0.000        &   1.438 $\pm$ 0.000           & 1.363 $\pm$ 0.001           \\
& Static NB-Po            &  0.663 $\pm$ 0.001      &  {\it 0.553 $\pm$ 0.002}&  1.208 $\pm$ 0.000       &  1.614 $\pm$ 0.002         &  0.625 $\pm$ 0.001         &  1.633 $\pm$ 0.001        &   {\it 1.343 $\pm$ 0.002     }& 1.257 $\pm$ 0.001           \\
& Static NB-NB            &  0.663 $\pm$ 0.000      &  0.620 $\pm$ 0.003      &  1.197 $\pm$ 0.000       &  1.730 $\pm$ 0.003         &  0.580 $\pm$ 0.001         &  1.605 $\pm$ 0.000        &   1.365 $\pm$ 0.001           & 1.290 $\pm$ 0.001           \\
& EWMA NB-Po              &  0.720 $\pm$ 0.001      &  0.751 $\pm$ 0.005      &  1.207 $\pm$ 0.000       &  1.541 $\pm$ 0.002         &  0.649 $\pm$ 0.001         &  1.668 $\pm$ 0.000        &   1.435 $\pm$ 0.002           & 1.358 $\pm$ 0.001           \\
& EWMA NB-NB              &  0.708 $\pm$ 0.001      &  0.764 $\pm$ 0.002      &  1.207 $\pm$ 0.000       &  1.540 $\pm$ 0.001         &  0.649 $\pm$ 0.001         &  1.668 $\pm$ 0.001        &   1.436 $\pm$ 0.002           & 1.358 $\pm$ 0.001           \\
& RNN G-Po                &  0.396 $\pm$ 0.005      &  {\bf 0.447 $\pm$ 0.005}&  1.346 $\pm$ 0.001       &  {\bf 1.375 $\pm$ 0.024   }&  {\bf 0.544 $\pm$ 0.005}   &  1.759 $\pm$ 0.002        &   {\bf 1.062 $\pm$ 0.004}     & {\bf 0.996 $\pm$ 0.006}     \\
& RNN G-NB                &  0.401 $\pm$ 0.006      &  0.452 $\pm$ 0.009      &  1.347 $\pm$ 0.002       &  1.408 $\pm$ 0.028         &  0.550 $\pm$ 0.016         &  1.761 $\pm$ 0.007        &   1.074 $\pm$ 0.005           & {\bf 1.015 $\pm$ 0.008}     \\
& RNN NB-Po               &  {\bf 0.388 $\pm$ 0.002}&  0.458 $\pm$ 0.003      &  1.349 $\pm$ 0.001       &  1.448 $\pm$ 0.036         &  0.561 $\pm$ 0.006         &  1.763 $\pm$ 0.003        &   {\bf 1.068 $\pm$ 0.001}     & 1.021 $\pm$ 0.008           \\
& RNN NB-NB               &  {\bf 0.385 $\pm$ 0.001}&  {\bf 0.448 $\pm$ 0.004}&  1.350 $\pm$ 0.006       &  1.465 $\pm$ 0.064         &  0.565 $\pm$ 0.036         &  1.765 $\pm$ 0.014        &   {\bf 1.068 $\pm$ 0.004}     & 1.026 $\pm$ 0.027           \\
\cline{1-10}
\multirow{16}{*}{\textbf{Auto}}
& All Zeros               &  N/A                    &  N/A                    &  0.785                   &  0.922                     &  1.000                     &  2.000                    &   9.618                       & 1.820                       \\
& Croston    \cCro        &  N/A                    &  N/A                    &  0.847                   &  0.841                     &  0.536                     &  1.077                    &   7.881                       & 1.477                       \\
& SBA        \cSBA        &  N/A                    &  N/A                    &  {\bf 0.846             }&  {\bf 0.835               }&  {\bf 0.529               }&  1.081                    &   7.868                       & {\bf 1.468                 }\\
& TSB        \cTSB        &  N/A                    &  N/A                    &  0.852                   &  0.857                     &  0.552                     &  1.079                    &   8.000                       & 1.501                       \\
& Static G-Po    \cCro    &  2.383 $\pm$ 0.002      &  {\bf 1.527 $\pm$ 0.001}&  0.848 $\pm$ 0.000       &  0.845 $\pm$ 0.000         &  0.540 $\pm$ 0.001         &  1.074 $\pm$ 0.000        &   {\bf 7.842 $\pm$ 0.004     }& 1.479 $\pm$ 0.001           \\
& Static G-NB    \cSny    &  {\bf 2.121 $\pm$ 0.000}&  2.277 $\pm$ 0.004      &  0.944 $\pm$ 0.000       &  1.182 $\pm$ 0.002         &  0.755 $\pm$ 0.000         &  1.136 $\pm$ 0.000        &   8.439 $\pm$ 0.003           & 1.828 $\pm$ 0.002           \\
& EWMA G-Po      \cShen   &  2.503 $\pm$ 0.008      &  1.574 $\pm$ 0.002      &  0.861 $\pm$ 0.000       &  0.872 $\pm$ 0.000         &  0.586 $\pm$ 0.000         &  1.088 $\pm$ 0.000        &   8.144 $\pm$ 0.010           & 1.525 $\pm$ 0.000           \\
& EWMA G-NB               &  2.330 $\pm$ 0.002      &  1.605 $\pm$ 0.001      &  0.861 $\pm$ 0.000       &  0.873 $\pm$ 0.000         &  0.586 $\pm$ 0.000         &  1.088 $\pm$ 0.000        &   8.134 $\pm$ 0.005           & 1.526 $\pm$ 0.000           \\
& Static NB-Po            &  2.335 $\pm$ 0.003      &  {\bf 1.521 $\pm$ 0.001}&  {\bf 0.840 $\pm$ 0.000} &  {\bf 0.825 $\pm$ 0.000   }&  {\bf 0.516 $\pm$ 0.000   }&  {\it 1.066 $\pm$ 0.000  }&   {\bf 7.809 $\pm$ 0.023     }& {\bf 1.452 $\pm$ 0.001}     \\
& Static NB-NB            &  {\bf 2.109 $\pm$ 0.002}&  2.271 $\pm$ 0.006      &  0.943 $\pm$ 0.000       &  1.167 $\pm$ 0.000         &  0.743 $\pm$ 0.001         &  1.136 $\pm$ 0.000        &   8.465 $\pm$ 0.009           & 1.809 $\pm$ 0.000           \\
& EWMA NB-Po              &  2.493 $\pm$ 0.001      &  1.575 $\pm$ 0.001      &  0.861 $\pm$ 0.000       &  0.871 $\pm$ 0.000         &  0.585 $\pm$ 0.000         &  1.088 $\pm$ 0.000        &   8.156 $\pm$ 0.016           & 1.524 $\pm$ 0.000           \\
& EWMA NB-NB              &  2.333 $\pm$ 0.003      &  1.606 $\pm$ 0.001      &  0.861 $\pm$ 0.000       &  0.872 $\pm$ 0.001         &  0.586 $\pm$ 0.001         &  1.089 $\pm$ 0.001        &   8.156 $\pm$ 0.008           & 1.526 $\pm$ 0.000           \\
& RNN G-Po                &  2.395 $\pm$ 0.020      &  1.649 $\pm$ 0.010      &  0.848 $\pm$ 0.004       &  0.857 $\pm$ 0.008         &  0.548 $\pm$ 0.014         &  {\bf 1.061 $\pm$ 0.001  }&   8.725 $\pm$ 0.016           & 1.492 $\pm$ 0.008           \\
& RNN G-NB                &  2.158 $\pm$ 0.028      &  1.834 $\pm$ 0.014      &  0.901 $\pm$ 0.008       &  1.001 $\pm$ 0.024         &  0.674 $\pm$ 0.036         &  1.076 $\pm$ 0.004        &   8.814 $\pm$ 0.053           & 1.630 $\pm$ 0.031           \\
& RNN NB-Po               &  2.411 $\pm$ 0.036      &  1.649 $\pm$ 0.005      &  0.851 $\pm$ 0.008       &  0.863 $\pm$ 0.017         &  0.554 $\pm$ 0.020         &  {\bf 1.062 $\pm$ 0.001  }&   8.634 $\pm$ 0.018           & 1.497 $\pm$ 0.016           \\
& RNN NB-NB               &  2.119 $\pm$ 0.009      &  1.892 $\pm$ 0.004      &  0.896 $\pm$ 0.004       &  0.981 $\pm$ 0.012         &  0.636 $\pm$ 0.013         &  1.076 $\pm$ 0.006        &   8.951 $\pm$ 0.015           & 1.605 $\pm$ 0.014           \\
\cline{1-10}
\multirow{16}{*}{\textbf{RAF}}
& All Zeros               &  N/A                    &  N/A                    &  0.785                   &  {\bf 0.578               }&  1.000                     &  2.000                    &   16.786                      & {\bf 1.423                 }\\
& Croston    \cCro        &  N/A                    &  N/A                    &  1.494                   &  1.048                     &  0.845                     &  1.949                    &   16.545                      & 1.777                       \\
& SBA        \cSBA        &  N/A                    &  N/A                    &  1.494                   &  1.040                     &  0.846                     &  1.950                    &   {\bf 16.543                }& 1.770                       \\
& TSB        \cTSB        &  N/A                    &  N/A                    &  1.494                   &  {\bf 0.932               }&  0.881                     &  1.963                    &   17.731                      & {\bf 1.710                 }\\
& Static G-Po    \cCro    &  1.312 $\pm$ 0.000      &  2.878 $\pm$ 0.008      &  1.494 $\pm$ 0.000       &  1.088 $\pm$ 0.000         &  0.842 $\pm$ 0.004         &  1.948 $\pm$ 0.000        &   16.557 $\pm$ 0.019          & 1.818 $\pm$ 0.000           \\
& Static G-NB    \cSny    &  1.287 $\pm$ 0.000      &  {\bf 2.354 $\pm$ 0.001}&  {\bf 1.490 $\pm$ 0.000} &  1.564 $\pm$ 0.001         &  {\bf 0.726 $\pm$ 0.003   }&  {\bf 1.936 $\pm$ 0.000  }&   {\bf 16.541 $\pm$ 0.018    }& 1.922 $\pm$ 0.001           \\
& EWMA G-Po      \cShen   &  1.339 $\pm$ 0.000      &  3.094 $\pm$ 0.006      &  1.494 $\pm$ 0.000       &  1.185 $\pm$ 0.001         &  0.863 $\pm$ 0.001         &  1.945 $\pm$ 0.000        &   16.657 $\pm$ 0.015          & 1.915 $\pm$ 0.000           \\
& EWMA G-NB               &  1.320 $\pm$ 0.000      &  2.782 $\pm$ 0.005      &  1.494 $\pm$ 0.000       &  1.185 $\pm$ 0.001         &  0.863 $\pm$ 0.002         &  1.945 $\pm$ 0.000        &   16.663 $\pm$ 0.007          & 1.925 $\pm$ 0.001           \\
& Static NB-Po            &  1.324 $\pm$ 0.000      &  3.299 $\pm$ 0.002      &  1.494 $\pm$ 0.000       &  1.280 $\pm$ 0.000         &  0.816 $\pm$ 0.002         &  1.941 $\pm$ 0.000        &   16.607 $\pm$ 0.015          & 1.956 $\pm$ 0.000           \\
& Static NB-NB            &  {\it 1.285 $\pm$ 0.000}&  2.448 $\pm$ 0.000      &  {\bf 1.488 $\pm$ 0.000} &  1.949 $\pm$ 0.003         &  {\bf 0.665 $\pm$ 0.002   }&  {\bf 1.926 $\pm$ 0.000  }&   16.596 $\pm$ 0.021          & 2.099 $\pm$ 0.001           \\
& EWMA NB-Po              &  1.299 $\pm$ 0.004      &  3.118 $\pm$ 0.003      &  1.494 $\pm$ 0.000       &  1.184 $\pm$ 0.000         &  0.856 $\pm$ 0.001         &  1.945 $\pm$ 0.000        &   16.666 $\pm$ 0.013          & 1.912 $\pm$ 0.001           \\
& EWMA NB-NB              &  1.291 $\pm$ 0.002      &  2.786 $\pm$ 0.006      &  1.493 $\pm$ 0.000       &  1.184 $\pm$ 0.000         &  0.859 $\pm$ 0.002         &  1.946 $\pm$ 0.000        &   16.668 $\pm$ 0.023          & 1.921 $\pm$ 0.001           \\
& RNN G-Po                &  {\bf 1.277 $\pm$ 0.001}&  2.592 $\pm$ 0.021      &  1.495 $\pm$ 0.000       &  1.217 $\pm$ 0.022         &  0.798 $\pm$ 0.005         &  1.946 $\pm$ 0.001        &   16.625 $\pm$ 0.007          & 1.825 $\pm$ 0.012           \\
& RNN G-NB                &  {\bf 1.278 $\pm$ 0.001}&  {\bf 2.407 $\pm$ 0.023}&  1.495 $\pm$ 0.000       &  1.183 $\pm$ 0.013         &  0.799 $\pm$ 0.002         &  1.949 $\pm$ 0.000        &   16.630 $\pm$ 0.006          & 1.763 $\pm$ 0.002           \\
& RNN NB-Po               &  {\bf 1.278 $\pm$ 0.002}&  2.893 $\pm$ 0.029      &  1.493 $\pm$ 0.000       &  1.407 $\pm$ 0.018         &  0.778 $\pm$ 0.005         &  1.938 $\pm$ 0.001        &   16.595 $\pm$ 0.010          & 1.964 $\pm$ 0.018           \\
& RNN NB-NB               &  {\bf 1.278 $\pm$ 0.002}&  2.499 $\pm$ 0.005      &  1.494 $\pm$ 0.000       &  1.297 $\pm$ 0.015         &  0.776 $\pm$ 0.004         &  1.943 $\pm$ 0.001        &   16.614 $\pm$ 0.004          & 1.837 $\pm$ 0.006           \\
% \cline{1-10}
% \multirow{16}{*}{\textbf{UCI}}
% & All Zeros               &  N/A                    &  N/A                    &  0.785                   &  {\bf 2.836               }&  1.000                     &  2.000                    &   7.661                       & {\bf 3.413                 }\\
% & Croston    \cCro        &  N/A                    &  N/A                    &  1.284                   &  3.112                     &  0.714                     &  1.735                    &   7.456                       & 3.466                       \\
% & SBA        \cSBA        &  N/A                    &  N/A                    &  1.283                   &  3.107                     &  0.709                     &  1.737                    &   7.460                       & 3.462                       \\
% & TSB        \cTSB        &  N/A                    &  N/A                    &  {\bf 1.267             }&  {\bf 3.046}               &  0.733                     &  1.730                    &   {\it 7.430                 }& {\bf 3.409                 }\\
% & Static G-Po    \cCro    &  2.059 $\pm$ 0.000      &  3.043 $\pm$ 0.006      &  1.287 $\pm$ 0.000       &  3.174 $\pm$ 0.002         &  0.714 $\pm$ 0.002         &  1.739 $\pm$ 0.000        &   7.488 $\pm$ 0.001           & 3.514 $\pm$ 0.002           \\
% & Static G-NB    \cSny    &  {\it 2.054 $\pm$ 0.000}&  {\it 3.041 $\pm$ 0.003}&  1.279 $\pm$ 0.000       &  3.286 $\pm$ 0.002         &  0.655 $\pm$ 0.002         &  {\it 1.729 $\pm$ 0.001  }&   7.458 $\pm$ 0.001           & 3.467 $\pm$ 0.002           \\
% & EWMA G-Po      \cShen   &  {\it 2.054 $\pm$ 0.001}&  3.079 $\pm$ 0.005      &  1.286 $\pm$ 0.000       &  3.232 $\pm$ 0.002         &  0.719 $\pm$ 0.001         &  1.732 $\pm$ 0.000        &   7.490 $\pm$ 0.001           & 3.548 $\pm$ 0.002           \\
% & EWMA G-NB               &  {\bf 2.043 $\pm$ 0.001}&  3.126 $\pm$ 0.004      &  1.287 $\pm$ 0.000       &  3.234 $\pm$ 0.001         &  0.726 $\pm$ 0.001         &  1.735 $\pm$ 0.000        &   7.494 $\pm$ 0.001           & 3.555 $\pm$ 0.000           \\
% & Static NB-Po            &  2.059 $\pm$ 0.000      &  3.121 $\pm$ 0.004      &  1.288 $\pm$ 0.000       &  3.384 $\pm$ 0.001         &  0.698 $\pm$ 0.001         &  1.757 $\pm$ 0.000        &   7.526 $\pm$ 0.002           & 3.585 $\pm$ 0.001           \\
% & Static NB-NB            &  2.059 $\pm$ 0.000      &  3.249 $\pm$ 0.001      &  1.282 $\pm$ 0.000       &  3.710 $\pm$ 0.014         &  {\it 0.667 $\pm$ 0.001   }&  1.749 $\pm$ 0.000        &   7.504 $\pm$ 0.001           & 3.596 $\pm$ 0.003           \\
% & EWMA NB-Po              &  2.120 $\pm$ 0.002      &  3.068 $\pm$ 0.004      &  1.285 $\pm$ 0.000       &  3.254 $\pm$ 0.002         &  0.731 $\pm$ 0.001         &  {\it 1.729 $\pm$ 0.000  }&   7.501 $\pm$ 0.002           & 3.568 $\pm$ 0.001           \\
% & EWMA NB-NB              &  2.061 $\pm$ 0.000      &  3.113 $\pm$ 0.006      &  1.285 $\pm$ 0.000       &  3.254 $\pm$ 0.001         &  0.736 $\pm$ 0.000         &  1.731 $\pm$ 0.000        &   7.503 $\pm$ 0.001           & 3.574 $\pm$ 0.001           \\
% & RNN G-Po                &  2.054 $\pm$ 0.004      &  2.929 $\pm$ 0.003      &  1.281 $\pm$ 0.000       &  3.384 $\pm$ 0.015         &  0.682 $\pm$ 0.006         &  1.703 $\pm$ 0.004        &   {\bf 7.402 $\pm$ 0.007     }& 3.551 $\pm$ 0.010           \\
% & RNN G-NB                &  {\bf 2.040 $\pm$ 0.003}&  {\bf 2.871 $\pm$ 0.006}&  1.280 $\pm$ 0.001       &  3.495 $\pm$ 0.056         &  0.695 $\pm$ 0.011         &  {\bf 1.685 $\pm$ 0.004  }&   {\bf 7.368 $\pm$ 0.007     }& 3.602 $\pm$ 0.026           \\
% & RNN NB-Po               &  2.081 $\pm$ 0.002      &  2.937 $\pm$ 0.004      &  1.277 $\pm$ 0.001       &  3.371 $\pm$ 0.008         &  {\bf 0.644 $\pm$ 0.004   }&  1.712 $\pm$ 0.001        &   7.429 $\pm$ 0.005           & 3.532 $\pm$ 0.005           \\
% & RNN NB-NB               &  2.063 $\pm$ 0.005      &  {\bf 2.918 $\pm$ 0.016}&  {\bf 1.273 $\pm$ 0.001} &  3.463 $\pm$ 0.036         &  {\bf 0.633 $\pm$ 0.005   }&  {\bf 1.694 $\pm$ 0.004  }&   7.404 $\pm$ 0.007           & 3.560 $\pm$ 0.016           \\
% \cline{1-10}
% \multirow{16}{*}{\textbf{M5}}
% & All Zeros               &  N/A                    &  N/A                    &  0.785 --                &  1.298 --                  &  1.000 --                  &  2.000 --                 &   3.852 --                    & 1.730 --                    \\
% & Croston    \cCro        &  N/A                    &  N/A                    &  1.088 --                &  1.378 --                  &  0.596 --                  &  1.429 --                 &   2.299 --                    & 1.370 --                    \\
% & SBA        \cSBA        &  N/A                    &  N/A                    &  1.088 --                &  1.359 --                  &  0.590 --                  &  1.436 --                 &   2.280 --                    & 1.364 --                    \\
% & TSB        \cTSB        &  N/A                    &  N/A                    &  1.060 --                &  1.320 --                  &  0.598 --                  &  1.430 --                 &   2.213 --                    & 1.323 --                    \\
% & Static G-Po    \cCro    &  2.059 $\pm$ 0.000      &  1.093 $\pm$ 0.000      &  0.730 $\pm$ 0.000       &  1.357 $\pm$ 0.000         &  0.616 $\pm$ 0.000         &  1.471 $\pm$ 0.000        &   2.453 $\pm$ 0.000           & 1.414 $\pm$ 0.000           \\
% & Static G-NB    \cSny    &  {\it 2.054 $\pm$ 0.000}&  1.250 $\pm$ 0.000      &  1.192 $\pm$ 0.001       &  1.538 $\pm$ 0.000         &  0.532 $\pm$ 0.000         &  1.458 $\pm$ 0.000        &   3.255 $\pm$ 0.001           & 1.520 $\pm$ 0.000           \\
% & EWMA G-Po      \cShen   &  {\it 2.054 $\pm$ 0.001}&  1.031 $\pm$ 0.000      &  0.667 $\pm$ 0.000       &  1.400 $\pm$ 0.000         &  0.593 $\pm$ 0.000         &  1.419 $\pm$ 0.000        &   2.301 $\pm$ 0.000           & 1.377 $\pm$ 0.000           \\
% & EWMA G-NB               &  {\bf 2.043 $\pm$ 0.001}&  1.015 $\pm$ 0.000      &  0.664 $\pm$ 0.000       &  1.400 $\pm$ 0.000         &  0.593 $\pm$ 0.000         &  1.419 $\pm$ 0.000        &   2.301 $\pm$ 0.000           & 1.378 $\pm$ 0.000           \\
% & Static NB-Po            &  2.059 $\pm$ 0.000      &  1.378 $\pm$ 0.000      &  0.786 $\pm$ 0.000       &  1.631 $\pm$ 0.000         &  0.615 $\pm$ 0.000         &  1.531 $\pm$ 0.000        &   3.040 $\pm$ 0.002           & 1.529 $\pm$ 0.000           \\
% & Static NB-NB            &  2.059 $\pm$ 0.000      &  1.384 $\pm$ 0.000      &  1.550 $\pm$ 0.001       &  2.050 $\pm$ 0.000         &  0.569 $\pm$ 0.000         &  1.514 $\pm$ 0.000        &   3.578 $\pm$ 0.001           & 1.728 $\pm$ 0.000           \\
% & EWMA NB-Po              &  2.120 $\pm$ 0.002      &  1.055 $\pm$ 0.000      &  0.663 $\pm$ 0.000       &  1.447 $\pm$ 0.000         &  0.593 $\pm$ 0.000         &  1.402 $\pm$ 0.000        &   2.306 $\pm$ 0.001           & 1.398 $\pm$ 0.000           \\
% & EWMA NB-NB              &  2.061 $\pm$ 0.000      &  1.032 $\pm$ 0.000      &  0.661 $\pm$ 0.000       &  1.448 $\pm$ 0.000         &  0.593 $\pm$ 0.000         &  1.403 $\pm$ 0.000        &   2.308 $\pm$ 0.000           & 1.399 $\pm$ 0.000           \\
% & RNN G-Po                &  2.054 $\pm$ 0.004      &  2.929 $\pm$ 0.003      &  1.281 $\pm$ 0.000       &  3.384 $\pm$ 0.015         &  0.682 $\pm$ 0.006         &  1.703 $\pm$ 0.004        &   {\bf 7.402 $\pm$ 0.007     }& 3.551 $\pm$ 0.010           \\
% & RNN G-NB                &  {\bf 2.040 $\pm$ 0.003}&  {\bf 2.871 $\pm$ 0.006}&  1.280 $\pm$ 0.001       &  3.495 $\pm$ 0.056         &  0.695 $\pm$ 0.011         &  {\bf 1.685 $\pm$ 0.004  }&   {\bf 7.368 $\pm$ 0.007     }& 3.602 $\pm$ 0.026           \\
% & RNN NB-Po               &  2.081 $\pm$ 0.002      &  2.937 $\pm$ 0.004      &  1.277 $\pm$ 0.001       &  3.371 $\pm$ 0.008         &  {\bf 0.644 $\pm$ 0.004   }&  1.712 $\pm$ 0.001        &   7.429 $\pm$ 0.005           & 3.532 $\pm$ 0.005           \\
% & RNN NB-NB               &  2.063 $\pm$ 0.005      &  {\bf 2.918 $\pm$ 0.016}&  {\bf 1.273 $\pm$ 0.001} &  3.463 $\pm$ 0.036         &  {\bf 0.633 $\pm$ 0.005   }&  {\bf 1.694 $\pm$ 0.004  }&   7.404 $\pm$ 0.007           & 3.560 $\pm$ 0.016           \\
\bottomrule
\end{tabular}
}
\end{adjustwidth}
% }
% \end{adjustbox}
\end{sidewaystable}


\begin{sidewaystable}
\label{tab:results_dtrp_2}
\centering
\caption{Experiment results for discrete-time models with UCI and M5 sets}
% \begin{adjustbox}{angle=90}
\begin{adjustwidth}{0in}{0in}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{3cm}p{8cm}cccccccc}
\toprule
Data Set  & Model         &     P50 Loss            &         P90 Loss        &  MAAPE                   &   MASE                     &  MAPE                      &             sMAPE         &   RMSE                        & RMSSE                       \\
\midrule
\multirow{16}{*}{\textbf{UCI}}
& All Zeros               &  N/A                    &  N/A                    &  {\bf 0.785             }&  {\bf 2.836               }&  1.000                     &  2.000                    &   7.661                       & {\bf 3.413                 }\\
& Croston    \cCro        &  N/A                    &  N/A                    &  1.284                   &  3.112                     &  0.714                     &  1.735                    &   7.456                       & 3.466                       \\
& SBA        \cSBA        &  N/A                    &  N/A                    &  1.283                   &  3.107                     &  0.709                     &  1.737                    &   7.460                       & 3.462                       \\
& TSB        \cTSB        &  N/A                    &  N/A                    &  {\bf 1.267             }&  {\bf 3.046}               &  0.733                     &  1.730                    &   {\it 7.430                 }& {\bf 3.409                 }\\
& Static G-Po    \cCro    &  2.059 $\pm$ 0.000      &  3.043 $\pm$ 0.006      &  1.287 $\pm$ 0.000       &  3.174 $\pm$ 0.002         &  0.714 $\pm$ 0.002         &  1.739 $\pm$ 0.000        &   7.488 $\pm$ 0.001           & 3.514 $\pm$ 0.002           \\
& Static G-NB    \cSny    &  {\it 2.054 $\pm$ 0.000}&  {\it 3.041 $\pm$ 0.003}&  1.279 $\pm$ 0.000       &  3.286 $\pm$ 0.002         &  0.655 $\pm$ 0.002         &  {\it 1.729 $\pm$ 0.001  }&   7.458 $\pm$ 0.001           & 3.467 $\pm$ 0.002           \\
& EWMA G-Po      \cShen   &  {\it 2.054 $\pm$ 0.001}&  3.079 $\pm$ 0.005      &  1.286 $\pm$ 0.000       &  3.232 $\pm$ 0.002         &  0.719 $\pm$ 0.001         &  1.732 $\pm$ 0.000        &   7.490 $\pm$ 0.001           & 3.548 $\pm$ 0.002           \\
& EWMA G-NB               &  {\bf 2.043 $\pm$ 0.001}&  3.126 $\pm$ 0.004      &  1.287 $\pm$ 0.000       &  3.234 $\pm$ 0.001         &  0.726 $\pm$ 0.001         &  1.735 $\pm$ 0.000        &   7.494 $\pm$ 0.001           & 3.555 $\pm$ 0.000           \\
& Static NB-Po            &  2.059 $\pm$ 0.000      &  3.121 $\pm$ 0.004      &  1.288 $\pm$ 0.000       &  3.384 $\pm$ 0.001         &  0.698 $\pm$ 0.001         &  1.757 $\pm$ 0.000        &   7.526 $\pm$ 0.002           & 3.585 $\pm$ 0.001           \\
& Static NB-NB            &  2.059 $\pm$ 0.000      &  3.249 $\pm$ 0.001      &  1.282 $\pm$ 0.000       &  3.710 $\pm$ 0.014         &  {\it 0.667 $\pm$ 0.001   }&  1.749 $\pm$ 0.000        &   7.504 $\pm$ 0.001           & 3.596 $\pm$ 0.003           \\
& EWMA NB-Po              &  2.120 $\pm$ 0.002      &  3.068 $\pm$ 0.004      &  1.285 $\pm$ 0.000       &  3.254 $\pm$ 0.002         &  0.731 $\pm$ 0.001         &  {\it 1.729 $\pm$ 0.000  }&   7.501 $\pm$ 0.002           & 3.568 $\pm$ 0.001           \\
& EWMA NB-NB              &  2.061 $\pm$ 0.000      &  3.113 $\pm$ 0.006      &  1.285 $\pm$ 0.000       &  3.254 $\pm$ 0.001         &  0.736 $\pm$ 0.000         &  1.731 $\pm$ 0.000        &   7.503 $\pm$ 0.001           & 3.574 $\pm$ 0.001           \\
& RNN G-Po                &  2.071 $\pm$ 0.007      &  {\bf 2.906 $\pm$ 0.004}&  1.281 $\pm$ 0.000       &  3.411 $\pm$ 0.013         &  0.676 $\pm$ 0.006         &  {\bf 1.699 $\pm$ 0.002  }&   {\bf 7.393 $\pm$ 0.004     }& 3.562 $\pm$ 0.010           \\
& RNN G-NB                &  {\bf 2.039 $\pm$ 0.001}&  {\bf 2.870 $\pm$ 0.004}&  1.277 $\pm$ 0.001       &  3.445 $\pm$ 0.029         &  0.669 $\pm$ 0.011         &  {\bf 1.686 $\pm$ 0.003  }&   {\bf 7.368 $\pm$ 0.004     }& 3.566 $\pm$ 0.012           \\
& RNN NB-Po               &  2.086 $\pm$ 0.005      &  2.937 $\pm$ 0.005      &  1.275 $\pm$ 0.001       &  3.463 $\pm$ 0.004         &  {\bf 0.637 $\pm$ 0.004   }&  1.702 $\pm$ 0.002        &   7.423 $\pm$ 0.004           & 3.573 $\pm$ 0.001           \\
& RNN NB-NB               &  2.062 $\pm$ 0.003      &  2.923 $\pm$ 0.004      &  {\bf 1.271 $\pm$ 0.001} &  3.452 $\pm$ 0.057         &  {\bf 0.618 $\pm$ 0.005   }&  {\bf 1.699 $\pm$ 0.003  }&   7.417 $\pm$ 0.004           & 3.539 $\pm$ 0.018           \\
\cline{1-10}
\multirow{16}{*}{\textbf{M5}}
& All Zeros               &  N/A                    &  N/A                    &  0.785 --                &  {\bf 1.298}               &  1.000 --               &  2.000 --               &  3.852 --                 & 1.730 --                      \\
& Croston    \cCro        &  N/A                    &  N/A                    &  1.088 --                &  1.378 --                  &  0.596 --               &  1.429 --               &  2.299 --                 & 1.370 --                      \\
& SBA        \cSBA        &  N/A                    &  N/A                    &  1.088 --                &  1.359 --                  &  0.590 --               &  1.436 --               &  {\bf 2.280}              & 1.364 --                      \\
& TSB        \cTSB        &  N/A                    &  N/A                    &  {\bf 1.060 }            &  {\bf 1.320}               &  0.598 --               &  1.430 --               &  {\bf 2.213}              & {\bf 1.323}                   \\
& Static G-Po    \cCro    &  1.093 $\pm$ 0.000      &  0.730 $\pm$ 0.000      &  1.099 $\pm$ 0.000       &  1.357 $\pm$ 0.000         &  0.616 $\pm$ 0.000      &  1.471 $\pm$ 0.000      &  2.453 $\pm$ 0.000        & 1.414 $\pm$ 0.000             \\
& Static G-NB    \cSny    &  1.250 $\pm$ 0.000      &  1.192 $\pm$ 0.001      &  1.086 $\pm$ 0.000       &  1.538 $\pm$ 0.000         &  {\bf 0.532 $\pm$ 0.000}&  1.458 $\pm$ 0.000      &  3.255 $\pm$ 0.001        & 1.520 $\pm$ 0.000             \\
& EWMA G-Po      \cShen   &  {\bf 1.031 $\pm$ 0.000}&  0.667 $\pm$ 0.000      &  1.085 $\pm$ 0.000       &  1.400 $\pm$ 0.000         &  0.593 $\pm$ 0.000      &  1.419 $\pm$ 0.000      &  2.301 $\pm$ 0.000        & 1.377 $\pm$ 0.000             \\
& EWMA G-NB               &  1.015 $\pm$ 0.000      &  0.664 $\pm$ 0.000      &  1.085 $\pm$ 0.000       &  1.400 $\pm$ 0.000         &  0.593 $\pm$ 0.000      &  1.419 $\pm$ 0.000      &  2.301 $\pm$ 0.000        & 1.378 $\pm$ 0.000             \\
& Static NB-Po            &  1.378 $\pm$ 0.000      &  0.786 $\pm$ 0.000      &  1.116 $\pm$ 0.000       &  1.631 $\pm$ 0.000         &  0.615 $\pm$ 0.000      &  1.531 $\pm$ 0.000      &  3.040 $\pm$ 0.002        & 1.529 $\pm$ 0.000             \\
& Static NB-NB            &  1.384 $\pm$ 0.000      &  1.550 $\pm$ 0.001      &  1.099 $\pm$ 0.000       &  2.050 $\pm$ 0.000         &  0.569 $\pm$ 0.000      &  1.514 $\pm$ 0.000      &  3.578 $\pm$ 0.001        & 1.728 $\pm$ 0.000             \\
& EWMA NB-Po              &  1.055 $\pm$ 0.000      &  0.663 $\pm$ 0.000      &  {\bf 1.081 $\pm$ 0.000} &  1.447 $\pm$ 0.000         &  0.593 $\pm$ 0.000      &  {\bf 1.402 $\pm$ 0.000}&  2.306 $\pm$ 0.001        & 1.398 $\pm$ 0.000             \\
& EWMA NB-NB              &  1.032 $\pm$ 0.000      &  {\bf 0.661 $\pm$ 0.000}&  {\bf 1.081 $\pm$ 0.000} &  1.448 $\pm$ 0.000         &  0.593 $\pm$ 0.000      &  1.403 $\pm$ 0.000      &  2.308 $\pm$ 0.000        & 1.399 $\pm$ 0.000             \\
& RNN G-Po                &  {\bf 1.028 $\pm$ 0.016}&  {\bf 0.654 $\pm$ 0.006}&  1.085 $\pm$ 0.003       &  1.384 $\pm$ 0.011         &  {\bf 0.585 $\pm$ 0.014}&  1.421 $\pm$ 0.008      &  2.387 $\pm$ 0.046        & {\bf 1.360 $\pm$ 0.004}       \\
& RNN G-NB                &  1.111 $\pm$ 0.059      &  0.916 $\pm$ 0.152      &  1.092 $\pm$ 0.009       &  1.589 $\pm$ 0.141         &  0.625 $\pm$ 0.051      &  {\bf 1.399 $\pm$ 0.005}&  3.025 $\pm$ 0.234        & 1.512 $\pm$ 0.108             \\
& RNN NB-Po               &  1.041 $\pm$ 0.017      &  0.675 $\pm$ 0.009      &  1.091 $\pm$ 0.004       &  1.421 $\pm$ 0.021         &  0.586 $\pm$ 0.004      &  1.444 $\pm$ 0.013      &  2.412 $\pm$ 0.047        & 1.372 $\pm$ 0.005             \\
& RNN NB-NB               &  1.063 $\pm$ 0.035      &  0.721 $\pm$ 0.030      &  1.090 $\pm$ 0.007       &  1.437 $\pm$ 0.014         &  0.596 $\pm$ 0.044      &  1.433 $\pm$ 0.011      &  2.644 $\pm$ 0.114        & 1.387 $\pm$ 0.018             \\
\bottomrule
\end{tabular}
}
% \end{adjustwidth}
% }
% \end{adjustbox}
\end{sidewaystable}

